How can classical multidimensional scaling go wrong?

Given a matrix $D$ describing the pairwise dissimilarities of a data set, a common task is to embed the data points into Euclidean space. The classical multidimensional scaling (cMDS) algorithm is a widespread method to do this. However, theoretical analysis of the robustness of the algorithm and an in-depth analysis of its performance on non-Euclidean metrics is lacking. In this paper, we derive a formula, based on the eigenvalues of a matrix obtained from $D$, for the Frobenius norm of the difference between $D$ and the metric $D_{\text{cmds}}$ returned by cMDS. This error analysis leads us to the conclusion that when the derived matrix has a significant number of negative eigenvalues, then $\|D-D_{\text{cmds}}\|_F$, after initially decreasing, will eventually increase as we increase the dimension. Hence, counterintuitively, the quality of the embedding degrades as we increase the dimension. We empirically verify that the Frobenius norm increases as we increase the dimension for a variety of non-Euclidean metrics. We also show on several benchmark datasets that this degradation in the embedding results in the classification accuracy of both simple (e.g., 1-nearest neighbor) and complex (e.g., multi-layer neural nets) classifiers decreasing as we increase the embedding dimension. Finally, our analysis leads us to a new efficiently computable algorithm that returns a matrix $D_l$ that is at least as close to the original distances as $D_t$ (the Euclidean metric closest in $\ell_2$ distance). While $D_l$ is not metric, when given as input to cMDS instead of $D$, it empirically results in solutions whose distance to $D$ does not increase when we increase the dimension and the classification accuracy degrades less than the cMDS solution.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

==> intro.tex <==
\section{Introduction}
\label{sec:introduction}

\begin{enumerate}
	\item What is MDS?
	\item What's the classical algorithm for solving it? cMDS
	\item What's wrong with MDS as a problem? and cMDS as an algorithm? MDS is difficult to solve, folks have created a zillion variants (by generalizing and changing the objective function). cMDS doesn't actually solve the MDS problem. cMDS as an algorithm is not particularly robust to outliers or perturbations.
	\item EXCEPT no one has analyzed just how non-robust it is! Despite a zillion alternatives, heuristics, and (approximation) algorithms. Cayton and Dasgupta have some heuristic arguments as to how non-robust cMDS and MDS can be in their Robust Euclidean Embeddings paper. They also point out the difference between the optimization problem that cMDS solves and that of MDS.
	\item we seek to quantify this difference -- just how big a problem is this? Are these MDS alternatives and generalizations any better than cMDS? When? What about if we start with data not from a Euclidean space? What if we specify a low-rank or a high-rank?
\end{enumerate}


Learning an embedding into Euclidean space is a standard pre or post processing step in many data pipelines. One of the most common ways this is done, is using the classical Multidimensional Scaling Algorithm (cMDS). For cMDS, given a distance matrix $D_p$, we learn an embedding $X_{cmds}$ whose columns are vectors representing the embedding by solving the following problem. 
\[
    X_{cmds} = \argmin_{X \in \mathbb{R}^{r \times n}} \left\|X^TX - \left(\frac{-V(D\circ D)V}{2}\right)\right\|,
\]
where $V$ is the centering matrix given by $V := I - \frac{1}{n}J$. Here $I$ is the identity matrix and $J$ is the matrix of all ones.  

Now given an embedding $X$, let $EDM(X)$ be the corresponding Euclidean distance matrix. That is, 
\[
    EDM(X)_{ij} = \|X_i - X_j\|^2,
\]
where $X_i,X_j$ are the $i$th and $j$th columns of $X$. Then we see that $D_{cmds} := EDM(X_{cmds})$ is not the solution to the following problem. 
\begin{equation}
\label{eq:mds}    \min_{D = EDM(X), X \in \mathbb{R}^{r \times n}} \|D - (Dp \circ Dp)\|^2.
\end{equation}
The problem in Equation \ref{eq:mds} is the true Multidimensional Scaling problem. Hence we see that the cMDS algorithm is just an approximation algorithm for the MDS problem. While it is possible to solve the true MDS problem exactly (it is a convex optimization problem), it is computational expensive to do so. Thus, the question that we are interested in as follows. Let $D_{t}$ be the solution to the problem in Equation \ref{eq:mds}, then we are interested in understanding the quantity $err := \|D_t - D_{cmds}\|$. In particular, can we predict when $err$ is small without having to compute $D_t$. Doing so provide practitioners with multiple advantages. 

\begin{enumerate}
    \item If $err$ is guaranteed to be small, then we can use the cMDS algorithm without having to worry about loss in quality of the solution. 
    \item If $err$ is big, we can now make an informed decision about whether benefits of the speed of cMDS algorithm versus the quality of the solution. 
    \item Understanding when $err$ is big helps us design algorithms to approximate the solution to MDS problem that perform better when cMDS fails. 
    \item Understanding $err$ is also the first step in rigorously quantifying the robustness of the cMDS algorithm.
\end{enumerate}


==> intro2.tex <==
%!TEX root = main.tex
\section{Introduction}
\label{sec:introduction}
%Ideas for rewrite:
%
%\begin{enumerate}
%    \item So people had issues of what is MDS, with STRESS, SAMMOn stress etc. So idea to fix, instead calling it true MDS i think the literature is more commonly calls its metric mds. Cite this version, googling metric mds gives us many papers. Also we should define these other objectives (Stress, Sammon stress) and note that the trend for $\|D-Dcmds\|$ gives us the trend for all of the others. This way we frame the MDS problem and the issue better.
%    \item There is a big difference in the classification score for noisy MNIST (using the first 500 images of MNIST). I have currently run until dimension 75 -cmds: 34.4\%, tmds: 45.8, alg2+cmds: 51.2. The accuracy for alg2 + lower seems roughly constant, the accuracy for cmds seems to be falling.  For the Libras dataset I have results showing true does better than cmds on the downstream task of classification. Its reduced to 32\% and its best performance was at the dimension with the lowest error. 
%    \item Tried CIFAR10 - but everything did around 10\% (there are 10 classes). Now trying FashionMNIST. Similar trend for Fashion MNIST as well. 
%    \item We should clean up section 3.1. I think remove all of the explanation for how we derive the lower bound and just state and discuss the implications of theorem 1 part 1 and theorem 2. So remove the whole math computation. 
%    \item I can add in the proof for theorem 2. 
%\end{enumerate}


Multidimensional scaling (MDS) refers to a class of techniques for analyzing pairwise dissimilarities between arbitrary objects. The goal is to find an embedding of points
in a (usually) low dimensional space where the pairwise distances between these points
represent, as best as possible, the given pairwise distances between objects \cite{carroll1998multidimensional, borg2005modern}.
%represent, as best as possible, given pairwise distances as distances between points in lying in some (usually) low dimensional
%space
Apart from the
general usefulness of dimensionality reduction, MDS has been used in a wide
variety of applications including data visualization, data preprocessing,
network analysis, bioinformatics, %\cite{taguchi2005relational}
 and data
exploration.  Due to its long history and being well studied, MDS has many
variations such as nonmetric MDS \cite{shepard1962analysis,
shepard1962analysis2}, multi-way MDS \cite{kroonenberg2008applied}, multi-view
MDS \cite{bai2017multidimensional}, confirmatory or constrained MDS
\cite{heiser1983constrained}, etc. (See \cite{france2010two,
cox2008multidimensional} for surveys).

The basic MDS formulation involves minimizing an objective function over a space
of embeddings. There are two main objective functions associated with MDS: STRESS and STRAIN.
The STRAIN objective (see Equation \ref{eq:cmds} below) was introduced by Torgerson
\cite{torgerson1952}, whose algorithm to solve for this objective is now commonly referred to as the classical MDS algorithm (cMDS).
This algorithm first centers the squares of the given distance matrix and then uses
its spectral decomposition to extract the low dimensional embedding.
cMDS is one of the oldest and most popular methods for MDS, and its popularity is in part due to the fact that this decomposition is very fast and can scale to large 
matrices. The point set produced by cMDS, however, is not necessarily the point set whose Euclidean distance matrix is closest under say Frobenius norm to the input dissimilarity matrix. This type of objective is instead captured by STRESS, which comes in a variety of related forms. In particular, in this paper we consider the SSTRESS objective, shown in Equation \ref{eq:mds} below (and we remark below on its relation to other types of STRESS). There are algorithms to solve the SSTRESS objective, but the main drawback is that they are slow in comparison to cMDS (\cite{takane1977nonmetric,HAYDEN1988115,Qi2014}). Thus, many practitioners default to using cMDS and do not optimize for SSTRESS.

%(Edit this paragraph: keep same theme but get into Eucldiean vs. non-Euclidean. Talk about dimension. We don't know the right dimension, so the increase matters. Save discussion of lower bound and experiments for next paragraph)

In this paper, we shed light on the theoretical and practical differences
between optimizing for these two objectives. 
Specifically, let $err$ denote the value obtained by applying the SSTRESS objective function to the optimal STRAIN solution. 
Our main theorem, Theorem~\ref{thm:result}, decomposes $err$ into three components.
This decomposition gives insight into when and why cMDS can fail with respect to the SSTRESS objective. In particular, for Euclidean inputs, $err$ naturally decreases as the embedding dimension increases. For non-Euclidean inputs, however, our decomposition shows that after an initial decrease, counterintuitively $err$ can actually increase as the embedding dimension increases. 
%Moreover, this increase is predicted and described by one of the terms in our decomposition. 
This surprising increasing behavior is shown empirically on several real world data sets. 
In practice one may not know a priori what dimension to embed into, though might assume it suffices to embed into some sufficiently large dimension. Importantly, these results demonstrate that when using cMDS to embed into lower dimensions, choosing a dimension too large can actually increase error. Moreover, our decomposition can be used to quickly predict the dimension where this increase might occur. 

%We then provide downstream experiments (classification tasks) which show that it is better to optimize for SSTRESS than it is to optimize for Strain. Finally, using the insights from Theorem 1, we give a fast algorithm that computes a seed which, given as input to cMDS, results in a much lower error for SSTRESS and better classification accuracy.

%It should be noted that the Euclidean point set returned by cMDS is not necessarily the point set whose Euclidean distance matrix is closest (under Frobenius norm) to the input distance matrix....

%However, the simplicity and speed of cMDS comes at the cost of being
%a heuristic; it does not solve the true MDS problem (compare Equation \ref{eq:mds} to \ref{eq:cmds}). Furthermore, solving
%the true MDS problem is computationally expensive. A practitioner
%wants to know when she can use cMDS and when she cannot. 
%This leads to a few natural questions: (i) how bad can the cMDS solution be compared to the true solution? (ii) Under
%what conditions does cMDS perform well/poorly? (iii) Does the embedding dimension
%matter? (iv) What if the given (dis)similarity matrix does not come from points in a
%Euclidean space? (v) How robust is cMDS (compared to the true solution) to noisy data?

This degradation of the cMDS solution is of particular concern in relation to the robustness in the presence of noisy or missing data, as may often be the case for real world data. Several authors \cite{cayton2006robust, mandanas2016robust, forero2012sparsity} have proposed proposed variations to specifically address robustness with cMDS. However, our decomposition of $err$, suggests a novel approach. Specifically, by attempting to directly correct for the problematic term in our decomposition (which resulted in $err$ increasing with dimension) we produce a new lower bound solution. We show empirically that this lower bound corrects for $err$ increasing, both by itself and when used as a seed for cMDS. Crucially the running time of our new approach is comparable to cMDS, rather than the prohibitively expensive optimal SSTRES solution. Finally, and perhaps more importantly, we show that if we add noise or missing entries to real world data sets, then our new solution outperforms cMDS in terms of the downstream task of classification accuracy, under various classifiers.



%The observation that cMDS can perform poorly in the presence of noisy data is not new. In addition to the variations of MDS mentioned previously, several authors \cite{cayton2006robust, mandanas2016robust, forero2012sparsity} have proposed even more variations to specifically address robustness with cMDS. 
%Despite the widespread use of cMDS and the awareness of and variations to remedy non-robustness,
%even though this issue is well known,many variations to address it,
%awareness of these drawbacks of cMDS,
%Despite the widespread use of cMDS,
%there is, however, surprisingly little analysis of the above questions. \cite{cayton2006robust} give heuristic arguments that show cMDS is not robust for non-Euclidean distance matrices.
%Cayton and Dasgupta also discuss the large body of research on bounding the
%distortion of embeddings between various spaces. The work on bounding embedding distortion is motivated more by geometric and combinatorial concerns and does not address the above
%questions which come from a data analysis perspective.
%(Other previous work??)

%In this paper we answer these questions about cMDS by establishing theoretical and experimental results on its performance.

\textbf{Problem statements and contributions}

Given a dissimilarity matrix \( D \) whose entries are squared, here we consider the embedding producing the closest EDM to $D$ under Frobenius norm. Specifically, given an embedding $X$, $EDM(X)$ is the corresponding Euclidean distance matrix, that is 
\[
    \edm(X)_{ij} = \|X_i - X_j\|^2_F,
\]
where $X_i,X_j$ are the $i$th and $j$th columns of $X$. Then we are interested in the matrix, 
\begin{equation}
\label{eq:mds}   D_t := \argmin_{D' = EDM(X), X \in \mathbb{R}^{r \times n}} \|D' - D\|^2_F,
\end{equation}
Note that the reason we assume our dissimilarity matrix has squared entries is because the standard EDM definition uses squared entries (see further discussion of EDM's below). 
Equation~\ref{eq:mds} is a well studied objective \citep{takane1977nonmetric,HAYDEN1988115,Qi2014}, and is commonly referred to as SSTRESS. 
There are a number of similarly defined objectives. 
If one considers this objective when the matrix entries are not squared (i.e.\ $\sqrt{D'_{ij}}-\sqrt{D_{ij}}$), then it is referred to as STRESS. 
%Thus if $p$ is the exponent, then $p=1$ is STRESS, $p=2$ is SSTRESS, and more generally one can consider other values of $p$. 
If one further normalize each entry of the matrix difference by the input distance value (i.e.\ $(\sqrt{D'_{ij}}-\sqrt{D_{ij}})/\sqrt{D_{ij}}$) then it is called Sammon Stress. In this paper, we are less concerned with the differences between different types of Stress, and instead focus on how the cMDS solution behaves generally under a Stress type objective. Thus for simplicity we focus on SSTRESS.

As mentioned above, cMDS does not solve \ref{eq:mds} but instead solves for the following objective
\begin{equation} \label{eq:cmds}
    X_{\cmds} := \argmin_{X \in \mathbb{R}^{r \times n}} \left\|X^TX - 
            \left(\frac{-V D V}{2}\right)\right\|,
\end{equation}
where $V$ is the centering matrix given by 
\begin{equation}
	V := I - \frac{1}{n}J.
\label{eq:V_def}
\end{equation} 
Here $I$ is the identity matrix and $J$ is the matrix of all ones. This standard MDS objective was introduced in \cite{torgerson1952} and is commonly referred to as STRAIN.

%So we see that $D_{\cmds} := \edm(X_{\cmds})$ is not the solution to the true
%MDS problem but is only an approximation to it.
%The problem in Equation \ref{eq:mds} is the true Multidimensional Scaling problem. Hence we see that the cMDS algorithm is just an approximation algorithm for the MDS problem. While it is possible to solve the true MDS problem exactly (it is a convex optimization problem), it is computational expensive to do so.


Let $D_{\cmds} := \edm(X_{\cmds})$ and $D_{t}$ be the
solution to the problem in Equation \ref{eq:mds}. We are interested in
understanding the quantity 
\begin{equation}
	\err := \|D - D_{\cmds}\|.
\label{eq:err_def}
\end{equation}
Doing so will provide practitioners with multiple advantages and will guide the development of better algorithms. In particular, 

%Other common objective functions for the MDS problem as follows. 

%\textbf{Stress:} Want to find an embedding $X = \{x_1, \hdots, x_n\}$, such that if $r_{ij} = \|x_i-x_j\|$, then we want the embedding to minimize $\sum_{i,j} (r_{ij} - \sqrt{D_{ij}})^2$

%\textbf{Sammon Stress:} Here we want to minimize 
%\[
%    \frac{1}{\sum_{i < j} \sqrt{D_{ij}}} \sum_{i< j} \frac{(r_{ij}-\sqrt{D_{ij}})^2}{\sqrt{D_{ij}}}
%\]

%Note the quantity that we analyzing is $\sum_{i < j} (r_{ij}^2 - D_{ij})^2$. However, we will show that this quantity increases as the embedding dimension increases. In that case, if $D_{ij}$ are positive, then have that $(r^2_{ij}-D_{ij})^2$ increasing implies that $(r_{ij} - \sqrt{D_{ij}})^2$ also increases. Thus, our analysis gives us information about the performance of cMDS with respect to these other objectives as well. 

\begin{enumerate}[nosep]
	\item Understanding $\err$ is the first step in rigorously quantifying the robustness of the cMDS algorithm.
    \item If $\err$ is guaranteed to be small, then we can use the cMDS algorithm without having to worry about loss in quality of the solution. 
    \item If $\err$ is big, we can make an informed decision about the benefits of the speed of the cMDS algorithm versus the quality of the solution. 
    \item Understanding when $\err$ is big helps us design algorithms to approximate $D_t$ that perform better when cMDS fails. 
    
\end{enumerate}


% \remove{
% Learning an embedding into Euclidean space is a standard pre or post processing step in many data pipelines. One of the most common ways this is done, is using the classical Multidimensional Scaling Algorithm (cMDS). For cMDS, given a distance matrix $D_p$, we learn an embedding $X_{cmds}$ whose columns are vectors representing the embedding by solving the following problem. 

% cMDS solves the following problem.
% \[
%     X_{cmds} = \argmin_{X \in \mathbb{R}^{r \times n}} \left\|X^TX - \left(\frac{-V(D\circ D)V}{2}\right)\right\|,
% \]
% where $V$ is the centering matrix given by $V := I - \frac{1}{n}J$. Here $I$ is the identity matrix and $J$ is the matrix of all ones.  

% Now given an embedding $X$, let $EDM(X)$ be the corresponding Euclidean distance matrix. That is, 
% \[
%     EDM(X)_{ij} = \|X_i - X_j\|^2,
% \]
% where $X_i,X_j$ are the $i$th and $j$th columns of $X$. Then we see that $D_{cmds} := EDM(X_{cmds})$ is not the solution to the following problem. 
% \begin{equation}
% \label{eq:mds}    \min_{D = EDM(X), X \in \mathbb{R}^{r \times n}} \|D - (Dp \circ Dp)\|^2.
% \end{equation}
% The problem in Equation \ref{eq:mds} is the true Multidimensional Scaling problem. Hence we see that the cMDS algorithm is just an approximation algorithm for the MDS problem. While it is possible to solve the true MDS problem exactly (it is a convex optimization problem), it is computational expensive to do so. Thus, the question that we are interested in as follows. Let $D_{t}$ be the solution to the problem in Equation \ref{eq:mds}, then we are interested in understanding the quantity $err := \|D_t - D_{cmds}\|$. In particular, can we predict when $err$ is small without having to compute $D_t$. Doing so provide practitioners with multiple advantages. 
% }

% \begin{enumerate}[nosep]
%     \item If $\err$ is guaranteed to be small, then we can use the cMDS algorithm without having to worry about loss in quality of the solution. 
%     \item If $\err$ is big, we can now make an informed decision about whether benefits of the speed of cMDS algorithm versus the quality of the solution. 
%     \item Understanding when $\err$ is big helps us design algorithms to approximate the solution to MDS problem that perform better when cMDS fails. 
%     \item Understanding $\err$ is also the first step in rigorously quantifying the robustness of the cMDS algorithm.
% \end{enumerate}

The main contribution of our paper are as follows. 
\begin{enumerate}[nosep]
	\item We decompose the error in Equation~\ref{eq:err_def} into three terms that depend on the eigenvalues of a matrix obtained from $D$. Using this analysis, we show that there is a term that tells us that as we increase the dimension that we embed into, eventually, the error starts increasing. 
	\item We verify, using classification as a downstream task, that this increase in the error for cMDS results in the degradation of the quality of the embedding, as demonstrated by the classification accuracy decreasing. 
	\item Using this analysis, we provide an efficiently computable algorithm that returns a matrix $D_l$ such that if $D_t$ is the solution to Equation~\ref{eq:mds}, then $\|D_l - D\|_F \le \|D_t-D\|_F$, and empirically we see that $\|D_l-D_t\|_F \le \|D_{\cmds}-D_t\|_F$. 
	\item While $D_l$ is not metric, when given as input to cMDS instead of $D$, it results in solutions that are empirically better than the cMDS solution. This modified procedure results in a more natural decreasing of the error as the dimension increases and has better classification accuracy. 
\end{enumerate}

% \textcolor{red}{
% \begin{enumerate}
% 	\item What is MDS?
% 	\item What's the classical algorithm for solving it? cMDS
% 	\item What's wrong with MDS as a problem? and cMDS as an algorithm? MDS is difficult to solve, folks have created a zillion variants (by generalizing and changing the objective function). cMDS doesn't actually solve the MDS problem. cMDS as an algorithm is not particularly robust to outliers or perturbations.
% 	\item EXCEPT no one has analyzed just how non-robust it is! Despite a zillion alternatives, heuristics, and (approximation) algorithms. Cayton and Dasgupta have some heuristic arguments as to how non-robust cMDS and MDS can be in their Robust Euclidean Embeddings paper. They also point out the difference between the optimization problem that cMDS solves and that of MDS.
% 	\item we seek to quantify this difference -- just how big a problem is this? Are these MDS alternatives and generalizations any better than cMDS? When? What about if we start with data not from a Euclidean space? What if we specify a low-rank or a high-rank?
% \end{enumerate}
% }
